Lookout for Zombies: Mitigating Flush+Reload Attack on Shared Caches by Monitoring Invalidated Lines

OS-based page sharing is a commonly used optimization in modern systems to reduce memory footprint. Unfortunately, such sharing can cause Flush+Reload cache attacks, whereby a spy periodically flushes a cache line of shared data (using the clflush instruction) and reloads it to infer the access patterns of a victim application. Current proposals to mitigate Flush+Reload attacks are impractical as they either disable page sharing, or require application rewrite, or require OS support, or incur ISA changes. Ideally, we want to tolerate attacks without requiring any OS or ISA support and while incurring negligible performance and storage overheads. This paper makes the key observation that when a cache line is invalidated due to a Flush-Caused Invalidation (FCI), the tag and data of the invalidated line are still resident in the cache and can be used for detecting Flush-based attacks. We call lines invalidated due to FCI as Zombie lines. Our design explicitly marks such lines as Zombies, preserves the Zombie lines in the cache, and uses the hits and misses to Zombie lines to tolerate the attacks. We propose Zombie-Based Mitigation (ZBM), a simple hardware-based design that successfully guards against attacks by simply treating hits on Zombie-lines as misses to avoid any timing leaks to the attacker. We analyze the robustness of ZBM using three spy programs: attacking AES T-Tables, attacking RSA Square-and-Multiply, and Function Watcher (FW), and show that ZBM successfully defends against these attacks. Our solution requires negligible storage (4-bits per cache line), retains OS-based page sharing, requires no OS/ISA changes, and does not incur slowdown for benign applications.

==> memattacks.tex <==
\section{Appendix}
While this paper is focused on mitigating Flush+ Reload cache attacks using Zombie-lines, we observe that Zombies can also help in detecting other attacks that require repeated use of \texttt{clflush}. In this section, we discuss the application of Zombie-based detection to DRAM and cache coherence attacks (unfortunately, evaluating these is beyond our scope due to space limitations). Compared to naively counting flushes, counting flushes-on-zombies could lower the false-positives in attack detection -- as this can detect episodes of repeat flushes to the same line (common to such attacks).\ignore{ Evaluating these attacks is beyond the scope of this paper, due to space limitations.}

\subsection{Tolerating DRAM Timing Side-Channels} 
DRAMA~\cite{DramaRowbuffer} exploits DRAM row-buffer timing as a side-channel. This attack uses the timing difference between row-hit and row-miss to leak the access pattern. To execute at a sufficiently fast rate, the attack requires flush of the cache line in each iteration to ensure that the data is always read from memory. As these attacks incur frequent episodes of Zombie-Miss and then Flush-on-Zombie, we can count such episodes with dedicated hardware counters and detect a potential attack. When the counters cross a threshold, mitigation can be performed by switching to a closed-page policy.

\ignore{performance and power benefits of open-page policy in benign scenario.}

\subsection{Tolerating DRAM Row-Hammer Attacks}

Row-Hammer attacks~\cite{kim:isca14} flush two cache lines in each iteration, each corresponding to a different row in the same bank of DRAM. This causes frequent accesses to alternate rows, and a large number of row closures on the same rows within a short time-period. This injects faults in other neighbouring rows (due to faulty isolation in DRAM technology). Adversaries leverage this to inject bit-flips and modify access control bits in sensitive kernel data-structures, engineering illegal privilege escalation. While this attack can be mitigated by increasing the DRAM refresh rate\ignore{ from 64ms to 32ms/16ms}, such a solution incurs performance and power overheads. Instead, as these attacks incur frequent episodes of Zombie-Miss and then Flush-on-Zombie, detection is possible with dedicated hardware counters tracking these episodes. When the count exceeds a threshold, mitigation can be performed by increasing the DRAM refresh rate for a certain time period.

\subsection{Tolerating Coherence-Based Attacks}

OS-shared pages can leak information through the coherence status of their cached lines, as per recent attacks~\cite{yao:coherence}. Such attacks exploit the difference in cache access latency, based on whether the line is in Exclusive (\textit{E}) or Shared (\textit{S}) state. The spy first initializes the line to \textit{E}, then allows the victim to execute.  Later, by checking if the line is in \textit{S} (based on access latency), the spy can infer if the victim accessed it.

For this attack, re-initializing the line to \textit{E} is essential on each iteration: achieved with a {\texttt{clflush}} to invalidate the line, and a subsequent load to re-install it in \textit{E} (note: using stores to invalidate copies of lines leveraging coherence is not useful as that would unshare OS-shared pages). Hence, detecting episodes of repeated flush and reload to the same line, using hardware counters for Zombie-misses and Flushes-on-Zombies, can help detect such attacks. When the counts cross a threshold, mitigation can be activated in hardware by servicing  \textit{S} and \textit{E} accesses with similar (worst-case) latency.

\ignore{
\subsection{Tolerating DRAM Timing Attacks}


%Flush-based attacks allow the adversary to  control which lines can be accessed from memory. 

Recent memory attacks have used cache-line flushes to orchestrate fault-injection or memory-timing attacks. DRAMA~\cite{DramaRowbuffer} exploits DRAM row-buffer timing as a side-channel. This attack uses the timing difference between row-hit and row-miss to leak the access pattern. To execute at a sufficiently fast rate, the attack requires flush of the cache line in each iteration to ensure that the data is read from memory in each iteration. While this attack can be mitigated by switching to a closed-page policy, ideally, we would like to have the performance and power benefits of open-page policy and switch to closed-page policy only under attacks.  Our solution can detect DRAMA attacks, as these attacks incur frequent episodes of Zombie-Miss. We can dedicate a counter to keep track of the number of episodes of Zombie-Miss, and  when the number of such events exceed a threshold, mitigation can be performed by switching to a closed-page policy.

\subsection{Tolerating DRAM Row-Hammer Attacks}


Row-Hammer attacks~\cite{kim:isca14} flush two cache lines in each iteration, each corresponding to a different row in the same bank of DRAM memory (for example, Row-A and Row-B). This causes frequent access to the two rows, and large number of row closures on the same rows of memory within a short period of time. Such an attack injects faults in rows neighboring to the rows being accessed (due to faulty isolation in DRAM technology), and attempts to modify access control bits, to obtain higher privilege illegally. Row-Hammer attacks can be mitigated by reducing the DRAM refresh time from 64ms to 32ms/16ms; however, such a solution incurs performance and power overheads.  Our Zombie-based monitoring can detect Row-Hammer attacks, as these attacks incur frequent episodes of Zombie-Miss. We can dedicate a counter to keep track of the number of Zombie-Miss, and  when this number exceeds a threshold, mitigation can be performed by increasing the DRAM refresh rate for a certain time period.

%using policies described in Section~\ref{sec:os}.


\ignore{
An adversary can use flushing of shared lines to create alternative attacks to observe victim's access patterns. For example, Flush+Flush~\cite{FlushFlush} attacks use the variation in latency of the flush instruction, depending on whether the line is resident in the cache or not, to infer whether it was accessed by a victim. Such an attack can be mitigated using constant time implementation of clflush instruction. Furthermore, we can also use our insights about monitoring zombie lines to detect and mitigate such attacks. For example, for a Flush+Flush attack to be successful, a flush instruction must cause invalidation of a recently invalidated line (at least a few times). We can use the events of Flush operations to invalid-zombie lines to detect the Flush+Flush attacks and provide mitigation in the hardware or the OS.
}



\ignore{
\subsection{Mitigating Flush-Based Covert Channel Attacks}
}




\subsection{Tolerating Coherence-Based Attacks}
\label{sec:coherence_attacks}

We deem a line to be a zombie only if it gets invalidated due to a Flush, and invalidations due to coherence operations do not create zombie lines. Therefore, read-write sharing of data between different threads of a multi-threaded program (such as ping-pong on a spin lock) does not affect the zombie status of a line. Such read-write shared pages that belong to only one process are not the target of the cross-core Flush+Reload attacks, which try to leak information across two independent processes with only OS-shared pages in common. 


%(such attacks are not effective in our setup of a single chip with a shared L3)

Even though such OS-shared pages are used in a read-only mode by user processes, an attacker~\cite{yao:coherence} can use the coherence status of these lines to infer the access patterns in a multi-node system. Such attacks exploit the difference in cache latency, depending on whether the line is in Exclusive (E) or Shared (S) state. By initializing the line to state-E, the spy can infer an access by the victim, as the line would transition the line to S-state on a victim access.

Our solution can detect such coherence-based attacks. For such attacks, initializing the line to state-E is an essential component for each attack attempt, that is achieved by executing a {\texttt{clflush}} to invalidate the line, before a subsequent load to install the line in state-E. With our solution, the flush operation would mark the line as a zombie. Counting subsequent flushes to zombie lines can help detect the attack. It can then be mitigated in hardware by enforcing constant-time accesses independent of coherence state. 


}

==> old_todo.tex <==
Edit the backgorund paragarph on related work (identical as intro) -- SK

===

Flush to read‑only‑shared‑page, then Unshare: Indeed possible and in spirit of Section‑6
(Hardware detects + OS mitigates). <=== Final line in the conclusion?

====

SHARP restriction on clflush is not practical -- disables data dedup 


==> os.tex <==
\newpage
\section{Alternative Mitigation Policies Using OS}
\label{sec:os}

Thus far, we have focused on detection and mitigation of attacks entirely in hardware. However, our insight about using invalidated lines for detecting attack-like behavior can be used to enable alternative mitigation policies in OS as well. In this section, we discuss such a hybrid approach where hardware does the attack detection and the OS does the attack mitigation. 
%ng the attack.


\subsection{Zombie-Based Detection of Cross-Core Attacks}

For a successful cross-core attack using the Flush+Reload attack, there two conditions that must be met: (1) there must be a flush of a shared line (2) such invalidations must be followed by at-least one access to the line which brings the flushed line in the cache. For a cross-core attack to be successful, it is important that the above actions of flush and reload must happen from different cores at least some of the time. We leverage this behavior to identify the pair of applications that could be victim and spy in a cross-core attack. We call this mechanism {\em Zombie-Based Detection (ZBD).} Figure~\ref{fig:zbd} shows our hardware-based framework for ZBD.



\begin{figure}[htb] 
  	\centering
	\includegraphics[width=2.5 in]{FIGURES/zbd.eps}
	\caption{Zombie-Based Detection (ZBD) of Cross-Core Attacks (ADT counter overflow cause an interrupt for OS alarm).}
    \vspace{-0.1 in}
	\label{fig:zbd} 
\end{figure}


ZBD contains a hardware-based two-dimensional table of counters called the {\em Attack Detection Table (ADT)}.  The ADT counters are indexed on the x-axis by the core that caused the flush (Flushing-CoreID) and on the y-axis by core that incurred a miss on the invalid-zombie line (Zmiss-CoreID).  We equip each cache line in the cache to also store the ID of the {\em Flushing-CoreID }.  On a Zombie-Miss, we use the ID of the core that encountered the miss and the Flushing-CoreID stored in the zombie-line to increment the corresponding ADT counter. The diagonals of the ADT indicate flush and reload by the same core. For the cross-core attacks, we expect the non-diagonal entries to get incremented. When the non-diagonal entries reach a threshold (say maximum value of the counter), the ADT interrupts the OS and informs it of a possible Flush+Reload attack and provides the index of the ADT entry that caused the overflow. We use 4-bit counters and the hardware periodically (every 10ms) halves all the counters. For an 8-core system, ADT requires only 32 bytes.



%in the ADT table. For an 8-core system, the ADT requires an overhead of only 32 bytes.



\subsection{OS-Based Mitigation using ZBD}
%\vspace{-0.05in}
For the cross-core attack to be successful, it is necessary that both the victim and the spy processes are located in the same coherence domain (spatial sharing) and that they are scheduled concurrently (temporal sharing).  For OS-based mitigation policies, we target these requirements.  When the ZBD triggers the OS alarm (due to a non-diagonal ADT counters overflow), the OS first tries to identify the victim and the spy.  If the alarm was caused by a counter at co-ordinate (x,y) then x caused the flush of the lines and is identified as the spy, and "y" the victim.  Once the victim and spy processes are identified, then the OS can  provide either spatial isolation or temporal isolation between the victim and  spy, as shown in Figure~\ref{fig:os}. 






\begin{figure}[htb] 
  	\centering
%     \vspace{-0.1 in}
	\includegraphics[width=2.5in]{FIGURES/os.eps}
%	\vspace{-0.05 in}
    \caption{OS-Based Mitigation Using ZBD}
 %   \vspace{-0.15 in}
	\label{fig:os} 
\end{figure}

%\vspace{0.025 in}
    
\subsubsection{Spatial Isolation: Place in Different Domains}

A {\texttt{clflush}} instruction can remove a cache line only within the coherency domain. In systems, with a large number of independent machines (such as cloud computing), the scheduler could place the spy and the victim on different machines.

% with different memory domains.

\vspace{0.05 in}
    
\subsubsection{Temporal Isolation: Place in Different Time-slice}

Even if there is only one machine, the OS can still provide mitigation by scheduling the victim and the spy in different time-slices. This may reduce the throughput of the victim and the spy by up-to 50\%, however such slowdown will happen only when an attack is detected. Normal applications (without Flush+Reload) will not trigger the alarm and avoid slowdown.  

\vspace{0.05 in}

Figure~\ref{fig:osperf} shows the slowdown of aggregate system performance using temporal isolation for 103 workloads (100 benign + 3 attacks). Notice that there is no slowdown for the 100 benign workloads and loss of only 12-15\% system performance for the three workloads under attack with a spy. 

\begin{figure}[htb] 
%\begin{figure}[htb] 
  	\centering
    \vspace{-0.12 in}
   	\includegraphics[width=3.3in]{FIGURES/scurve_os.pdf}
    \vspace{-0.07 in}
	\caption{Slowdown for system performance for OS-based temporal isolation. Notice no slowdown for benign workloads. }
	\label{fig:osperf} 
  \vspace{-0.05 in}
\end{figure}
